NBNet: Noise Basis Learning for Image Denoising with Subspace Projection

In this paper, we introduce NBNet, a novel framework for image denoising. Unlike previous works, we propose to tackle this challenging problem from a new perspective: noise reduction by image-adaptive projection. Specifically, we propose to train a network that can separate signal and noise by learning a set of reconstruction basis in the feature space. Subsequently, image denosing can be achieved by selecting corresponding basis of the signal subspace and projecting the input into such space. Our key insight is that projection can naturally maintain the local structure of input signal, especially for areas with low light or weak textures. Towards this end, we propose SSA, a non-local subspace attention module designed explicitly to learn the basis generation as well as the subspace projection. We further incorporate SSA with NBNet, a UNet structured network designed for end-to-end image denosing. We conduct evaluations on benchmarks, including SIDD and DND, and NBNet achieves state-of-the-art performance on PSNR and SSIM with significantly less computational cost.

==> floats/fig_gauss_examples.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{pic/gauss_denoise.jpg}
    \caption{Results of Gaussian noise reduction when $\sigma = 70$.  (a)~Input (b) FFDNet. (c) VDN. (d) Ours. (e) Ground Truth}
    \label{fig:my_label}
\end{figure*}

==> floats/fig_more_results.tex <==
\begin{figure*}[t]
    \begin{center}
    %added by author2
    \begin{tabular}[t]{c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }}
    % \hspace{-2mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/69_noisy.jpg}& \hspace{-1.4mm}
    % \includegraphics[width=.14\textwidth]{Images/SIDD/RGB/SSID_0324_BM3D}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/69_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/69_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/69_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/69_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/69_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/72_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/72_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/72_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/72_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/72_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/72_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/129_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/129_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/129_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/129_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/129_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/129_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/169_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/169_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/169_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/169_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/169_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/169_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/179_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/179_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/179_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/179_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/179_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/179_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/289_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/289_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/289_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/289_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/289_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/289_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
     Noisy
    & VDN~\cite{yue2019variational}  & DANet~\cite{yue2020dual} & MIRNet~\cite{zamir2020learning} & Ours & Reference \\
    \end{tabular}
    \end{center}
    \vspace{-6mm}
    \caption{\small Denoising examples from SIDD}
    \label{fig:sidd more results1}
    %\vspace{-1.2em}
 \end{figure*}
 

==> floats/fig_more_results2.tex <==
\begin{figure*}[t]
    \begin{center}
    %added by author2
    \begin{tabular}[t]{c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }}
    % \hspace{-2mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/319_noisy.jpg}& \hspace{-1.4mm}
    % \includegraphics[width=.14\textwidth]{Images/SIDD/RGB/SSID_0324_BM3D}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/319_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/319_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/319_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/319_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/319_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/542_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/542_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/542_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/542_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/542_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/542_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/556_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/556_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/556_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/556_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/556_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/556_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/569_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/569_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/569_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/569_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/569_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/569_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/595_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/595_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/595_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/595_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/595_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/595_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
  
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/1121_noisy.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/1121_vdn.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/1121_da.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/1121_mir.jpg}& \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/1121_ssa.jpg}&  \hspace{-1.4mm}
    \includegraphics[width=.16\textwidth]{pic/SIDD_supp/1121_gt.jpg}
    \vspace{0.2mm}
    \\
    \vspace{0.5mm}
     Noisy
    & VDN~\cite{yue2019variational}  & DANet~\cite{yue2020dual} & MIRNet~\cite{zamir2020learning} & Ours & Reference \\
    \end{tabular}
    \end{center}
    \vspace{-6mm}
    \caption{\small Denoising examples from SIDD}
    \label{fig:sidd more results2}
    %\vspace{-1.2em}
 \end{figure*}
 

==> floats/fig_supp_basis.tex <==
\begin{figure*}[ht]
    \begin{subfigure}{}
    \centering
    \scalebox{1}{
    \begin{tabular}[b]{c@{ } c@{ }  }%\hspace{-2.4mm}
         \multirow{4}{*}{\includegraphics[width=.33\textwidth,valign=tl]{pic/basis/259_svd.jpg}} 
        &  \includegraphics[width=.152\textwidth,valign=t]{pic/basis/258_noisy.jpg}
        
         
        \vspace{0.5mm}
    \\
        &  Noisy   \\
 
        &\includegraphics[width=.152\textwidth,valign=t]{pic/basis/259_gt.jpg}  
        
         \\
    
          Visualization of basis & Reference 
         \\
         \multicolumn{2}{c}{(a)}
         \\
    
    \end{tabular}}
    \end{subfigure}
    \begin{subfigure}{}
    \centering
    \scalebox{1}{
    \begin{tabular}[b]{c@{ } c@{ } 	}%\hspace{-2.4mm}
         \multirow{4}{*}{\includegraphics[width=.33\textwidth,valign=tl]{pic/basis/485_svd.jpg}} 
        &  \includegraphics[width=.152\textwidth,valign=t]{pic/basis/485_noisy.jpg}
        
         
        \vspace{0.5mm}
    \\
        &  Noisy   \\
 
        &\includegraphics[width=.152\textwidth,valign=t]{pic/basis/495_gt.jpg}  
        
         \\
    
          Visualization of basis & Reference 
         \\
         \multicolumn{2}{c}{(b)}
         \\
               
    \end{tabular}}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {(a) and (b) are basis visualization of different input image.
    } }
    \label{fig:basis vector visual supp1}
    
 \end{figure*}

==> floats/fig_supp_basis2.tex <==
\begin{figure}[b]
    \begin{center}
    \begin{subfigure}
    \begin{center}
    
    \tiny
    \scalebox{0.9}{
    \begin{tabular}[b]{c@{ } c@{ }  c@{ } c@{ } c@{ }	}%\hspace{-2.4mm}
         \multirow{4}{*}{\includegraphics[width=.32\textwidth,valign=tl]{pic/basis/485_svd.jpg}} 
        &  \includegraphics[width=.152\textwidth,valign=t]{pic/basis/485_noisy.jpg}
        
         
        \vspace{0.5mm}
    \\
        &  Noisy   \\
 
        &\includegraphics[width=.152\textwidth,valign=t]{pic/basis/495_gt.jpg}  
        
         \\
    
          Visualization of basis & Reference 
         \\
               
    \end{tabular}}
    \end{center}
    \end{subfigure}
    \end{center}
    \vspace{-6mm}
    \caption{\small {caption
    } }
    \label{fig:basis vector visual supp2}
    
 \end{figure}

==> floats/table_abl_modules.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ccc}
    \toprule
     & Method  & PSNR(dB)\\
    \midrule
    1 & UNet + Blocks + Nonlocal & - \\
    %\hline
    2 & UNet+ Blocks + Nonlocal(Bottom) & 39.69\\
    3 & Oktay~\emph{et al.}~\cite{oktay2018attention} & 39.68 \\
    %\hline
    4 & UNet+ Blocks + SSA(Dot Product) & 27.09 \\
    %\hline
    
    5 & UNet + Blocks + SSA(Projection) & 39.75 \\
    \bottomrule
    \end{tabular}
    \caption{Ablation study on convolutional blocks and SSA, '-' denotes non-convergence}
    \label{tab:abl study modules}
\end{table}
